A micro-mechanics based extension of the GTN continuum model accounting for random void distributions

Randomness in the void distribution within a ductile metal complicates quantitative modeling of damage following the void growth to coalescence failure process. Though the sequence of micro-mechanisms leading to ductile failure is known from unit cell models, often based on assumptions of a regular distribution of voids, the effect of randomness remains a challenge. In the present work, mesoscale unit cell models, each containing an ensemble of four voids of equal size that are randomly distributed, are used to find statistical effects on the yield surface of the homogenized material. A yield locus is found based on a mean yield surface and a standard deviation of yield points obtained from 15 realizations of the four-void unit cells. It is found that the classical GTN model very closely agrees with the mean of the yield points extracted from the unit cell calculations with random void distributions, while the standard deviation $\textbf{S}$ varies with the imposed stress state. It is shown that the standard deviation is nearly zero for stress triaxialities $T\leq1/3$, while it rapidly increases for triaxialities above $T\approx 1$, reaching maximum values of about $\textbf{S}/\sigma_0\approx0.1$ at $T \approx 4$. At even higher triaxialities it decreases slightly. The results indicate that the dependence of the standard deviation on the stress state follows from variations in the deformation mechanism since a well-correlated variation is found for the volume fraction of the unit cell that deforms plastically at yield. Thus, the random void distribution activates different complex localization mechanisms at high stress triaxialities that differ from the ligament thinning mechanism forming the basis for the classical GTN model. A method for introducing the effect of randomness into the GTN continuum model is presented, and an excellent comparison to the unit cell yield locus is achieved.

==> Statistics.tex <==
\section{Statistical analysis}
\label{S:4}
The reported von Mises equivalent stress and mean stress representing the material condition immediately after yielding are collected from all analyses conducted in this work and presented as yield surfaces in the stress space given by the mean and von Mises equivalent stresses $(\sigma_e,\sigma_m)$. The results are further treated  statistically. The basics for the statistical analysis are given in the following section. The known, homogeneous FCC distribution is omitted from the statistical analyses performed in this work, and only the randomly generated void configurations provide statistical data. 

\subsection{Statistics}
For each value of initial void volume fraction, $f_0$, and applied stress condition, given by $\rho$, considered in this work, the mean distance from origin in the von Mises equivalent stress space, mean stress space, $\mu$, is calculated following

\begin{equation}
\label{eq:meandist}
    \mu = \frac{1}{n}\sum_{i=1}^n x_i, 
\end{equation}
\noindent where $n$ is the total number of unit cells with different void configurations for each combination of $f_0$ and $\rho$ considered, and $x_i$ is the distance from origin of the $i$th unit cell. The standard deviation of the mean distance is given as 

\begin{equation}
\label{eq:STD}
    \mathbf{S} = \sqrt{\frac{1}{n-1}\sum_{i=1}^n\abs{x_i-\mu}^2},
\end{equation}
\noindent while the standard error of mean, $\mathbf{SEM}$, is given as
\begin{equation}
\label{eq:SEM}
    \mathbf{SEM}=\frac{\mathbf{S}}{\sqrt{n}}.
\end{equation}

The standard error of mean can be interpreted as a measure for the dispersion of sample means around the population mean, where the population mean is given by Eq. \eqref{eq:meandist}.

\subsection{Homogenised yield surface for random, porous isotropic materials}
\label{sec:Gurson}
A homogenised yield criterion accounting for the statistical variations stemming from the different void distribution is proposed to reproduce the results from the unit cell analyses. The homogenised model used in this work takes as basis the Gurson yield surface \cite{gurson1977}, which reads

\begin{equation}
\label{eq:Gurson}
    \Phi = \frac{\sigma_e^2}{\sigma_0^2}+2q_1f_0 \text{cosh}\left[\frac{3}{2}q_2\frac{\sigma_m}{\sigma_0}\right]-\left(1+(q_1f_0)^2\right),
\end{equation}

\noindent where $\sigma_e$ is the von Mises equivalent stress, $\sigma_0$ is the yield stress of the matrix material, $\sigma_m$ is the mean stress, and $f_0$ is the initial void volume fraction. The factors introduced by Tvergaard \cite{tvergaard1981} are set to $q_1=1.5$ and $q_2=1$. As both the von Mises equivalent stress and the mean stress enter explicitly into the Gurson yield criteria in Eq. \eqref{eq:Gurson}, the yield surface spanning over the entire range of positive stress triaxialities in the $(\sigma_e, \sigma_m)$ stress space, is readily obtained. 

The expression for the Gurson yield surface given in Eq. \eqref{eq:Gurson} can be interpreted as a standard equation for a circle given by $x^2+y^2=r^2$. The first term of Eq. \eqref{eq:Gurson} gives the position along the vertical axis and the second term of Eq. \eqref{eq:Gurson} the position along the horizontal axis in a coordinate system defined by $(\sigma_e,\sigma_m)$. The last term of Eq. \eqref{eq:Gurson} determines the radius of the circle. To scale the radius of the yield surface in accordance with the standard deviation for the given $f_0$ and $\rho$, the proposition is to multiply $(1\pm S)^2$ with the last term, updating Eq. \eqref{eq:Gurson} to now reads 

\begin{equation}
\label{eq:GursonS}
    \Phi = \frac{\sigma_e^2}{\sigma_0^2}+2q_1f_0 \text{cosh}\left[\frac{3}{2}q_2\frac{\sigma_m}{\sigma_0}\right]-\left(1\pm \mathbf{S}\right)^2\left(1+(q_1f_0)^2\right),
\end{equation}
\noindent where $\mathbf{S}$ is the standard deviation given by interpolation of Eq. \eqref{eq:STD} over the range of applied stress conditions ($\rho$) considered in this work.

\subsection{Characterisation of deformation mechanism}
To determine the mechanism of plastic deformation, macroscopic plastic deformation or localisation, a plastic index has been defined. The plastic index, $\mathbf{PI}$, is calculated based on the plastic volume of the unit cell and defined as 

\begin{equation}
\label{eq:PI}
    \mathbf{PI} = \frac{V_p}{V},
\end{equation}
\noindent where $V$ is the total volume of the unit cell elements and $V_p$ is the plastic volume of the unit cell, which is found through

\begin{equation}
\label{eq:Vp}
    V_p=\sum_{e}\beta V_e,
\end{equation}
\noindent where $\beta$ is a flag indicating whether yielding has ($\beta=1$) or has not ($\beta=0$) taken place for the Gauss points in the current element, $e$. Where $V_e$ is the element volume, given as

\begin{equation}
\label{eq:Ve}
    V_e = \sum_{i=1}^{n_g}\sum_{j=1}^{n_g}\sum_{k=1}^{n_g}W_i W_j W_k \norm{J},
\end{equation}
\noindent where $n_g$ is the total number of Gauss points (in each direction), $W_i$ are the weights of the Gauss points and $\norm{J}$ is the determinant of the Jacobian matrix. 

The plastic index provides a measure to define the manner in which a unit cell undergoes plastic deformation. For a large value of $\mathbf{PI}$, i.e. $\mathbf{PI}\rightarrow 1$, the plastic volume is close to the volume of the unit cell itself, indicating that the unit cell as a whole undergoes plastic deformation. The deformation mechanism may be referred to as macroscopic yielding. If the plastic index is low, a small volume of the cell undergoes plastic deformation, which indicates that localisation has occurred. 

